How to send a real number using a single bit (and some shared randomness)

We consider the fundamental problem of communicating an estimate of a real number $x\in[0,1]$ using a single bit. A sender that knows $x$ chooses a value $X\in\set{0,1}$ to transmit. In turn, a receiver estimates $x$ based on the value of $X$. We consider both the biased and unbiased estimation problems and aim to minimize the cost. For the biased case, the cost is the worst-case (over the choice of $x$) expected squared error, which coincides with the variance if the algorithm is required to be unbiased. We first overview common biased and unbiased estimation approaches and prove their optimality when no shared randomness is allowed. We then show how a small amount of shared randomness, which can be as low as a single bit, reduces the cost in both cases. Specifically, we derive lower bounds on the cost attainable by any algorithm with unrestricted use of shared randomness and propose near-optimal solutions that use a small number of shared random bits. Finally, we discuss open problems and future directions.

==> rebuttal.tex <==

Reviewer 1:

We thank the reviewer for the helpful comments.

Reviewer comment: A detailed definition of the biased case seems to be missing, I assume in the biased case the mean does not have to be x. 
Reply: the problem is defined at lines 86-92. Specifically, we write: 
"Our objective is to minimize the \emph{cost} that is defined as the \emph{worst-case expected squared error}, i.e., $\max_{x \in [0,1]} \mathbb E[(\widehat x - x)^2]$. Note that the worst-case is taken over the value of $x$ and the expectation is over the randomness of the algorithm. 
In the \emph{unbiased} setting, we additionally require $\mathbb E[\widehat x]=x$, in which case the cost becomes $\Var[\widehat x]$, i.e., the estimation variance."
That is, the biased case is the worst-case expected squared error without the additional requirement that the estimation is unbiased.

Reviewer comment: The paper doesn't not provide any related work and I am not sure if the authors are the first to consider the problem. 

Reply: We acknowledge we do not have a separate related works section, but we do discuss related work, including the basic rounding schemes (rounding, randomized rounding) and dithering.  To the best of our knowledge, this is the first work that formalizes the problem of sending a real number using a single bit and limited shared randomness. We cite prior work for subtractive dithering, the closest related problem, in lines 225-228 and compare ours with it.  Dithering, together with deterministic and randomized rounding, are the only approaches previously proposed.
Should we learn about other works relevant to our settings, we will be happy to cite and compare with them.

Reviewer comment: The algorithms without any randomness are quite straight-forward and the results are not surprising at all. 

Reply: as written in lines 60-63, the algorithms without shared randomness (randomized and deterministic rounding) are widely used in practice, and we do not claim to be the first to propose them. Instead, we provide them for completeness and as a baseline.  In particular, we show that in our cost model these are indeed optimal when no shared randomness is allowed.

Reviewer comment: The authors give lots and lots of estimations but no real intuition why the shared randomness is able to improve the estimations. Hence, the writing of the paper should be improved, and a comparison with related work should be added.

Reply: We provide several estimators as there are multiple specific scenarios to consider, and we tailor our approach to each variation. We tried to build the paper from the simpler estimators to more complex ones to provide intuition, explaining the steps and how they help reduce the cost.  We can readily add some high-level intuition, specifically that the shared randomness provides an additional mechanism to relate the input x, the output bit(s), and the resulting estimate.
 
Reviewer 2:

We thank the reviewer for the helpful comments.

Reviewer 3:

We thank the reviewer for the helpful comments.

Reviewer comment: Unfortunately, there are still some gaps between the upper and lower bounds. This is, in my opinion, the main weakness of this work.

Reply:  We agree that it would be interesting to obtain tighter bounds, and we are actively working on the problem.  Of course, it can be difficult to achieve tight bounds on new problems, and we want to formalize and introduce people to these problems so that they may work on them as well.  

